Beyond Probabilities: Unveiling the Misalignment in Evaluating Large Language Models

Large Language Models (LLMs) have demonstrated remarkable capabilities across various applications, fundamentally reshaping the landscape of natural language processing (NLP) research. However, recent evaluation frameworks often rely on the output probabilities of LLMs for predictions, primarily due to computational constraints, diverging from real-world LLM usage scenarios. While widely employed, the efficacy of these probability-based evaluation strategies remains an open research question. This study aims to scrutinize the validity of such probability-based evaluation methods within the context of using LLMs for Multiple Choice Questions (MCQs), highlighting their inherent limitations. Our empirical investigation reveals that the prevalent probability-based evaluation method inadequately aligns with generation-based prediction. Furthermore, current evaluation frameworks typically assess LLMs through predictive tasks based on output probabilities rather than directly generating responses, owing to computational limitations. We illustrate that these probability-based approaches do not effectively correspond with generative predictions. The outcomes of our study can enhance the understanding of LLM evaluation methodologies and provide insights for future research in this domain.

==> 3_setup.tex <==
\section{Empirical Evidence}

Evaluating LLM is hard

issue of free-text generation

Evaluating with another LLM, there might be some bias

Evaluating with human: non-scalable, and bias too (cite our paper)

Proxy to multiple choice classification: eval with OLG/OSP/OLP etc.

Issue: inconsistent with free-text generation.




Large language models (LLMs) are gaining increasing popularity in both academia and industry, owing to their unprecedented performance in various applications. As LLMs continue to play a vital role in both research and daily use, their evaluation becomes increasingly critical. However, evaluating such unprecedented powerful models present several emerging challenges.


\paragraph{The Curse of Evaluating Generated Text}
There is a long discussion on properly evaluating natural language generation models, as the quality of the generated content is conditioned on various factors. The subjective nature of what constitutes high-quality output complicates establishing universal assessment metrics. The models' ability to produce a diverse range of outputs makes it hard to quantify their novelty and relevance. Unlike supervised learning, there's often no clear ``correct'' answer or ground truth for comparison. 

\paragraph{LLM or Human Evaluation}


\paragraph{Multiple Choice Question as a Proxy}
